NativE: Multi-modal Knowledge Graph Completion in the Wild

Multi-modal knowledge graph completion (MMKGC) aims to automatically discover the unobserved factual knowledge from a given multi-modal knowledge graph by collaboratively modeling the triple structure and multi-modal information from entities. However, real-world MMKGs present challenges due to their diverse and imbalanced nature, which means that the modality information can span various types (e.g., image, text, numeric, audio, video) but its distribution among entities is uneven, leading to missing modalities for certain entities. Existing works usually focus on common modalities like image and text while neglecting the imbalanced distribution phenomenon of modal information. To address these issues, we propose a comprehensive framework NativE to achieve MMKGC in the wild. NativE proposes a relation-guided dual adaptive fusion module that enables adaptive fusion for any modalities and employs a collaborative modality adversarial training framework to augment the imbalanced modality information. We construct a new benchmark called WildKGC with five datasets to evaluate our method. The empirical results compared with 21 recent baselines confirm the superiority of our method, consistently achieving state-of-the-art performance across different datasets and various scenarios while keeping efficient and generalizable. Our code and data are released at https://github.com/zjukg/NATIVE

==> author.tex <==
\author{Yichi Zhang$^{1,2}$, Zhuo Chen$^{1,2}$, Lingbing Guo$^{1,2}$, Yajing Xu$^{1,2}$, Binbin Hu$^3$, Ziqi Liu$^3$\\ Wen Zhang$^{1,2}$ and Huajun Chen$^{1,2,4*}$}
\thanks{$*$ Corresponding author}
\affiliation{
    \institution{$^1$Zhejiang University \quad $^2$Zhejiang University-Ant Group Joint Laboratory of Knowledge Graph\\ $^3$Ant Group\quad $^4$Alibaba-Zhejiang University Joint Institute of Frontier Technology\\}
    \city{Hang Zhou}
    \country{China}
}
\email{{zhangyichi2022, huajunsir}@zju.edu.cn}

==> chapters/1-picture.tex <==
\begin{figure}
\centering
\subfigure[\vspace{8pt}Statistics of modalities in different MMKGs.]{
% 两张图合并成一张图
% 下标用latexit
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{cccccc}
\toprule
Dataset & Image & Text & Numeric & Audio & Video\\
\midrule
\textbf{WN9-IMG} \cite{xie_image-embodied_2017-IKRL}  & \cmark & \cmark & \xmark & \xmark & \xmark\\
\textbf{MMKG} \cite{DBLP:conf/esws/LiuLGNOR19-MMKG} & \cmark & \cmark & \cmark & \xmark & \xmark\\
\textbf{Richpedia} \cite{DBLP:journals/bdr/WangWQZ20-Richpedia} & \cmark & \cmark & \xmark & \xmark & \xmark\\
\textbf{MKG-W/Y} \cite{xu_relation-enhanced_2022-MMRNS} & \cmark & \cmark & \xmark & \xmark & \xmark\\
\textbf{Kuaipedia} \cite{DBLP:journals/corr/abs-2211-00732-KuaiPedia} & \cmark & \cmark & \xmark & \cmark & \cmark\\
\textbf{TIVA} \cite{DBLP:conf/mm/WangMCML023-TIVA} & \cmark & \cmark & \xmark & \cmark & \cmark\\
\textbf{MMpedia} \cite{DBLP:conf/semweb/WuWLZWDHLR23-MMpedia} & \cmark & \cmark & \xmark & \xmark & \xmark\\
\bottomrule
\end{tabular}
}
}
\\
\subfigure[Modality information distribution overall TIVA.]
{\includegraphics[width=0.95\columnwidth]{pictures/introduction.pdf}}
\vspace{-8pt}
  \caption{The diversity and imbalance nature in MMKGs. We report the modalities included in each MMKG in (a) and the statistical information about the modality information distribution across dataset/entity in TIVA in (b).}
  \label{figure::introduction}
\vspace{-16pt}
\end{figure}

==> chapters/5.6-table.tex <==
\begin{figure}
\centering
\subfigure[The distrubution histgram of the $\sigma(\zeta_r)$.]{\includegraphics[width=0.9\linewidth]{pictures/distribution.pdf}}
\\
\subfigure[Statistics of modalities in different MMKGs.]{
\resizebox{0.85\columnwidth}{!}{
\begin{tabular}{c|c}
\toprule
Modality  & Relations                                      \\
\midrule
Structure & GovType, Headquarter. SisterStation, SpokenIn  \\
Image     & (Film)Genre, Capital, Producer, Position       \\
Text      & Affiliation, Nationality, DeathPlace, IsPartOf \\
Numeric   & Location, Leader, LeaderName, LeaderParty \\
\bottomrule
\end{tabular}}
}
\vspace{-16pt}
\caption{The high-frequency relations can raise the weight of the corresponding modality on DB15K.}
\label{figure::distribution}
\vspace{-16pt}
\label{table::modality}
\end{figure}
